Reinforcement Learning for Bandit Neural Machine Translation with Simulated Human Feedback

Machine translation is a natural candidate problem for reinforcement learning from human feedback: users provide quick, dirty ratings on candidate translations to guide a system to improve. Yet, current neural machine translation training focuses on expensive human-generated reference translations. We describe a reinforcement learning algorithm that improves neural machine translation systems from simulated human feedback. Our algorithm combines the advantage actor-critic algorithm (Mnih et al., 2016) with the attention-based neural encoder-decoder architecture (Luong et al., 2015). This algorithm (a) is well-designed for problems with a large action space and delayed rewards, (b) effectively optimizes traditional corpus-level machine translation metrics, and (c) is robust to skewed, high-variance, granular feedback modeled after actual human behaviors.

==> background.tex <==
\subsection{Recurrent neural networks}

A recurrent neural network (RNN) is a neural architecture that is widely used to 
learn continuous representations of variable-length sequences.
Given a sequence $w = (w_1, \cdots, w_l)$, the network 
starts from an initial hidden vector $h_0$ and iterates through each token
to compute a hidden vector for each time step. 
The current hidden vector $h_t$ is computed by applying a non-linear 
transformation on the previous hidden vector $h_{t - 1}$ and current token $w_t$:
\begin{equation}
  h_t = f_{\theta}(h_{t - 1}, e(w_t))
\end{equation} where $e(.)$ is an embedding lookup function, and $f_{\theta}$
is a non-linear function (e.g. LSTM or GRU), 
 $\theta$ are the parameters of the network.

RNNs are building blocks of many more complex neural architectures. 

\subsection{Neural machine translation}

A neural machine translation (NMT) model consists of an encoder and a decoder, 
each of which is an RNN. 
It directly models the posterior distribution 
$P_{\theta}(y \mid x)$ of translating a source sentence $x = (x_1, \cdots, x_n)$ to
a target sentence $y = (y_1, \cdots, y_m)$:
\begin{equation}
  P_{\theta}(y \mid x) = \prod_{t = 1}^m P_{\theta}(y_t \mid y_{<t}, x)
\end{equation} where $y_{<t}$ are all tokens in the target sentence prior to $y_t$. 

Each disitribution $P_{\theta}(y \mid y_{<t}, x)$ is the output of a linear 
transformation followed by a softmax function on the decoder's output vector 
$\tilde{h}_t^{dec}$: 
\begin{equation}
\begin{split}
  P_{\theta}(y \mid y_{<t}, x) &= \mathrm{softmax}(W_s \ \tilde{h}_t^{dec}) \\
  \tilde{h}_{t}^{dec} &= \tanh (W_o [h_t^{dec}; c_t]) \\
  c_t &= \mathrm{attend}(h_i^{enc}, h_t^{dec})
\end{split}
\end{equation} where 
$[.;.]$ is the concatenation of two vectors, 
$\mathrm{attend}(.,.)$ is an attention mechanism,
\footnote{
In this work, we use the global attention mechanism \cite{Bahnadau,Luong}.}
$h_i^{enc}$ and $h_t^{dec}$ are the hidden vectors generated by the encoder
and the decoder, respectively.


During training, the encoder first encodes $x$ to a continuous
vector $\Phi(x)$, which is used as the initial hidden vector for the decoder. 
The decoder performs regular RNN operations to produce a sequence of hidden 
vectors:
\begin{equation}
\begin{split}
  h_0^{dec} &= \Phi(x) \\
  h_t^{dec} &= f_{\theta} 
  \left( h_{t - 1}^{dec}, \left[ \tilde{h}_t^{dec}; e(y_t) \right] \right)
\end{split}
\label{eqn:decoder}
\end{equation} where $e(.)$ is a word embedding lookup operation, 
\footnote{Feeding $\tilde{h}_t^{dec}$ to 
the next step is known as ``input feeding'' (CITE).} 

In a supervised learning framework, an NMT model is trained under the 
maximum log-likelihood objective:
\begin{equation}
\begin{split}
  \max_{\theta} \mathcal{L}_{sup}(\theta) &= 
  \max_{\theta} \mathbb{E}_{(x, y) \sim D_{tr}} 
  \left[ \log P_{\theta} \left( y \mid x \right) \right]
\end{split}
\end{equation} where $D_{tr}$ is the training set.  

At inference time,  the ground-truth token $y_t$ in Equation \ref{eqn:decoder} 
is replaced by the model's own prediction $\hat{y}_t$:
\begin{equation}
  \hat{y}_t = \arg \max_y P_{\theta}(y \mid \hat{y}_{<t}, x)
\end{equation}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "emnlp2017"
%%% End: 

